Modeling Complex Event Scenarios via Simple Entity-focused Questions

Event scenarios are often complex and involve multiple event sequences connected through different entity participants. Exploring such complex scenarios requires an ability to branch through different sequences, something that is difficult to achieve with standard event language modeling. To address this, we propose a question-guided generation framework that models events in complex scenarios as answers to questions about participants. At any step in the generation process, the framework uses the previously generated events as context, but generates the next event as an answer to one of three questions: what else a participant did, what else happened to a participant, or what else happened. The participants and the questions themselves can be sampled or be provided as input from a user, allowing for controllable exploration. Our empirical evaluation shows that this question-guided generation provides better coverage of participants, diverse events within a domain, comparable perplexities for modeling event sequences, and more effective control for interactive schema generation.

==> sec_data.tex <==
\section{Data Processing}\label{sec:data}


\begin{figure*}
\centering
\includegraphics[width=\textwidth]{images/pipeline-bold.jpg}
\caption{Data processing pipeline}
\label{fig:data}
\end{figure*}

Typical event language models are usually trained on sequences of events in an autoregressive manner. Our proposed framework generates events as \textit{answers} to \textit{questions} about entities from a given \textit{context}. Therefore, the system needs data points which are in form of \textit{(Context, Question, Answer)} tuples. 

To process data to have a collection of such tuples, we initially extract sequences of events from raw text, and then use these sequences to create \textit{(Context, Question, Answer)} tuples. These steps are described in more details in the following sections.

\subsection{OpenIE Event Extraction}
Given a document $D$, all its events can be extracted and concatenated to form a single sequence of events, $e_1,e_2,...e_n$ where each $e_i$ is an OpenIE event tuple. 
This sequence is later used to create \textit{(Context, Question, Answer)} tuples as described later, to be used for the guided event language modeling.


\subsection{Tuples Creation}
A guided event language model requires tuples of form $(C, Q, A)$, where $C$ is the given \textit{context} at each time step consisting of a set of discourse sequences; $Q$ is the \textit{question} that is asked regarding an entity in the context and finally $A$ is the \textit{answer}, an event in which the entity in question is present and plays the role specified by that question. 


Given a sequence of events $e_1,e_2,...e_n$ extracted from a single document $D$, we go through all events one-by-one and try to create as many tuples as possible as follows:

% \gd{add some notation to make this more formal/precise} 

First,\gd{reference the figure here, and have the notation align with labeled variable names in the figure} all the noun phrases $N_{e_t}$ of the event-in-question $e_t$ will be detected.
For each $np_i$ in $N_{e_t}$, two questions are automatically generated: what else did $\boldsymbol{np_i}$ do?\gd{following the DL book notation, I think you shouldn't bold this -- that refers to a vector. I think $N$ should be $\mathbf{n}$ instead and $np_i$ should be $n_i$} and what else happened to $\boldsymbol{np_i}$?

Starting from $e_{t+1}$, all the following events in the discourse are traversed to find the events that can be the answers to the generated questions regarding $np$s in $N_{e_t}$.
For each subsequent event, we initially extract all the noun phrases $N_{e_j}$ and their roles using a dependency parser. We also find all the coreferring clusters $Cls$\gd{this is confusing, it sounds like CLS token. I would also just use single-letter var names} from the document $D$ the sequences are extracted from. We then choose an event $e_j$ as the answer to a question $q_{np_i}$ if there exists an $np_k$ in $N_{e_j}$ which is in the same coreference cluster $c_{np_i}$ as the entity in question $np_i$ from $N_{e_t}$ and plays the same role (agent or theme).

If there is an event satisfying the above conditions in the sequence, then a new tuple will be added to the list of tuples $T$ with $(e_1,..,e_t)$ (all the events precedent to the event-in-question) as the context, $q_{r_{np_i}}$ as the question (where $r$ shows the type of question) and $e_j$ as the answer event.


The steps of this pipeline as shown in \hyperref[fig:data]{Figure 2} are described in more details in the following sections. 

% example: the police arrested the suspect on several charges
\paragraph{Noun phrase detection}
The first step in automatically creating a large collection of data tuples is detecting all the noun phrases within the OpenIE extracted events. 
We use the spaCy \cite{Honnibal_spaCy_Industrial-strength_Natural_2020} dependency parser to identify all the noun phrases within an event. 
Instead of using the OpenIE events for noun phrase detection, we use the original sentences each event is extracted from to increase the accuracy of this module.

Given an event $e_t$ and the corresponding sentence from which it is extracted, this module will extract all the noun phrases from the sentence but only keep the ones which are present in $e_t$ as set $N_{e_t}$. This set will be used as the inputs for the next part where questions are generated.

\paragraph{Question generation}
Questions in this setting are used to guide the system to focus on a specific entity and the role it plays in the scenario. 
% While there might be other approaches in doing so, we preferred using questions as this will be a more natural way to interact with the system.

For event $e_t$ and it set of noun phrases $N_{e_t}$, for each noun phrase $np_i$ in the set, two question in the form of \{what else did $\boldsymbol{np_i}$ do?, what else happened to $\boldsymbol{np_i}$?\} can be generated. These questions can be automatically asked for all the noun phrases in $N_{e_t}$ which have been already extracted in the previous step.

Once the questions are generated, the next step would be finding events from the sequence that can serve as the answers to these questions. To do this, we first need to identify the noun phrases within the subsequent events as well their dependency parses and then use this information to pick appropriate events as the answers.
  

\paragraph{Noun phrase dependency parsing}
The questions are aimed at a specific entity with a specific \textit{role} of being an agent or a theme. To find the event responses to these questions, not only do we have to detect the noun phrases in all subsequent events in the discourse, but we also need to know what role they have. 

We use the Spacy \cite{Honnibal_spaCy_Industrial-strength_Natural_2020} dependency parser to identify the roles $r_{np_k}$ of the noun phrases of each event $N_{e_j}$ for events that come after the event-in-question $e_t$.

Once we have the roles, we can look for the right events corresponding to the questions which do not only contain a noun phrase $np_k$ similar to $np_i$ (the noun phrase used in question), but also $r_{np_k}$ is the role specified in the question. 

\paragraph{Coreference resolution}
In many cases, the noun phrases in events-in-question might not be \textit{exactly} present in the subsequent events but there might be  entities from the same coreference clusters. To detect such cases and increase the coverage of our set, we initially use a coreference resolution system to identify the coreferring clusters within the document $D$ from which events are extracted from. These clusters are used to find the answer events.

Using coreferring entities, the events that can be served as answers to the questions regarding $e_t$ either include $np_i$ or its coreference.

\paragraph{Answer selection}
The final step in data processing pipeline is selecting the events as the answers to the questions. 

For each event in the discourse sequence $e_t$ and a question $q_{np_i}$ regarding a noun phrase in $N_{e_j}$, we choose an event $e_j$ as the answer to a question $q_{np_i}$ if: first, there exists an $np_k$ in $N_{e_j}$ which is in the same coreference cluster $c_{np_i}$ as the entity in question $np_i$ from $N_{e_t}$ and second, $np_k$ plays the same role (agent or theme) as $np_i$.

If an event satisfies the above conditions, then a new tuple will be added to the list of tuples $T$. The context $C$ is the events $(e_1,..,e_t)$ (all the events precedent to the event-in-question), $q_{r_{np_i}}$ is the question $Q$ (where $r$ shows the type of question and whether it looks for an agent or a theme) and $e_j$ is the answer event $A$.

There might be events in the discourse for which we can not find events to the questions regarding their noun phrases in the sequence. 
This might happen either due to the fact some of the noun phrases do not play any role in the scenario or some of the roles can not be applied to certain noun phrases. For such cases, the questions will be discarded.
If for all the questions regarding an event, no answer is found, we will add a (context, question, answer) tuple to the set in which the question is \textit{what happens next?} and the answer will be the immediate event in the discourse. 

% \input{alg}
